slash: A Technique for Static Configuration-Logic Identification

Researchers have recently devised tools for debloating software and detecting configuration errors. Several of these tools rely on the observation that programs are composed of an initialization phase followed by a main-computation phase. Users of these tools are required to manually annotate the boundary that separates these phases, a task that can be time-consuming and error-prone (typically, the user has to read and understand the source code or trace executions with a debugger). Because errors can impair the tool's accuracy and functionality, the manual-annotation requirement hinders the ability to apply the tools on a large scale. In this paper, we present a field study of 24 widely-used C/C++ programs, identifying common boundary properties in 96\% of them. We then introduce \textit{slash}, an automated tool that locates the boundary based on the identified properties. \textit{slash} successfully identifies the boundary in 87.5\% of the studied programs within 8.5\ minutes, using up to 4.4\ GB memory. In an independent test, carried out after \textit{slash} was developed, \textit{slash} identified the boundary in 85.7\% of a dataset of 21 popular C/C++ GitHub repositories. Finally, we demonstrate \textit{slash}'s potential to streamline the boundary-identification process of software-debloating and error-detection tools.

==> implementation.tex <==
\vspace{-0.2cm}
\section{\name Implementation}
\label{sec:implementation}
We implemented \name in C++, using LLVM-$12$~\cite{LLVM:CGO04}.
\name takes as input LLVM bitcode for the target program.
Such bitcode can be produced using one of the compiler wrappers that produce whole-program LLVM bitcode for an unmodified C/C++, e.g., WLLVM~\cite{TL:WLLVM}.% and GLLVM~\cite{TL:GLLVM}.

Depending on whether the analysis target is a command-line program or one that reads configuration options from a file, \name considers the formal parameters of \code{main} or the file-reading APIs, respectively, to be the tainted sources. \ma{@Philipp: if I remember correctly, we consider the main for all programs not the file-reading API??}
\ps{Yes. Both would work, but our experiments showed that only following \texttt{main}'s \texttt{argv} is already sufficient.}

\name employs \phasar~\cite{10.1007/978-3-030-17465-1_22} to perform taint analysis and constant propagation.
\phasar is built on top of LLVM and offers precise whole-program, flow-, context-, and alias-sensitive dataflow analyses implemented using the \textit{Interprocedural Finite Distributive Subset} (IFDS)~\cite{Reps:1995:PID:199448.199462} framework.
% \twr{
% Clarify why both IFDS and IDE are mentioned here?
% Is the taint analysis a multi-phase computation that uses IFDS for one or more phases and IDE for one or more phases?
% Otherwise, just mention one framework.
% }
% that are implemented in \phasar~\cite{10.1007/978-3-030-17465-1_22}.
% IFDS and IDE are conceptual frameworks that allow for solving arbitrary distributive data-flow analysis elegantly and efficiently.
% \phasar is built on top of LLVM.
It provides a number of helper analyses, such as (inter-procedural) control-flow, call-graph, points-to, and type-hierarchy analysis, which permit whole-program analysis to be carried out.

For computing strongly connected components and dominators, we use the Boost graph library~\cite{DBLP:books/daglib/0028062} (BGL) and LLVM, respectively.
% \phasar is a data-flow analysis framework that is built on top of LLVM.
% It provides infrastructure to solve static-analysis problems, providing its users with various generic data-flow implementations---including, among others, IFDS and IDE.
% It also provides a number of helper analyses, such as (inter-procedural) control-flow, call-graph, points-to, and type hierarchy analysis, which permit whole-program analysis to be carried out.

% The \phasar taint analysis produces a set of \neck candidates, which are then filtered using the procedures in  \Cref{alg:boundary-algorithm} from \Cref{sec:approach} to obtain the actual \neck of the application under analysis, if one exists.
%The basic block that represents the \neck is marked for further analysis using symbolic execution in \klee by introducing a call to a special function that has been artificially introduced by our algorithm.



% \ma{Any justification why we used \phasar instead of SVF?}

% \ps{I don't think this is necessary. It would have been as valid to use SVF for computing data flows.} \ma{I didn't get it, can you elaborate pls}
% There is no specific reason. We could have also used SVF. I don't think we need justification for using PhASAR.


==> listings/toy_wc_struct.tex <==
\begin{lstlisting}[style=CStyle, caption={A scaled-down version of the \texttt{wc} utility.},label={wc},escapechar=@]
struct Flags {
	char count_char;
	int count_lines; };
int total_lines = 0;
int total_chars = 0;
int main(int argc, char** argv){
	struct Flags *flag;
	flag = malloc(sizeof(struct Flags));
	flag->count_char = 0;
	flag->count_lines = 0;
	if (argc >= 2)
		for (int i = 1; i < argc; i++) {
			if (!strcmp(argv[i], "-c")) flag->count_char = 1;
			if (!strcmp(argv[i], "-l")) flag->count_lines = 1; 
		}
	else 
	    usage();
	char buffer[1024];
	while (fgets(buffer, 1024,stdin)){
		if (flag->count_char) total_chars += decodeChar(buffer);
		if (flag->count_lines) total_lines++;
	}
	if (flag->count_char) printf("\#Chars = \%d", total_chars);
	if (flag->count_lines) printf("#Lines = %d", total_lines);
}
\end{lstlisting}

==> notation.tex <==
\section{Terminology and Notation}
\label{sec:notation}
In this work, we consider the \neck-identification task as a vertex-cut graph-partitioning problem since the \neck constitutes an articulation point in the control-flow graph. 
% \nam{we should mention why - \neck as the vertex-cut?}
In this section, we introduce the terminology and notation for some of the fundamental concepts.
For a summary of notation, see Table~\ref{tab:notation}.

% it's not necessary that I need to keep all these definitions, for example, I may remove V_c and V_m
\begin{table}[!tb]
\centering
\caption{Summary of Notation}
\begin{tabular}{ll}
\hline
$G$ & Whole Program Graph \\
$V$ & The set of vertices in $G$\\
$E$ & The set of control-flow edges in $G$ \\
% $E_d$ & \makecell[l]{The set of data-flow edges in $G$ 
% } \\
$B$ & \neck of $G$ \\
$V_c$ & The set vertices in the Configuration logic \\
$V_m$ & The set vertices Main logic \\
$BP$ & The set of properties holds at the \neck \\
$H$ & Function annotates vertices contain config-hosting vars \\
$F$ & Function vertex $v$ holds the properties $BP$ \\
$\mu$ & Distance metric from the entry vertex to the \neck\\
 \hline
\end{tabular}
\label{tab:notation}
\end{table}

% Let $G=(V,E_c,E_d)$ denote an Inter-procedural Control-Flow Graph (ICFG) of a program $P$, where $V$ is the set of vertices and $E_c\subseteq V\times V$ is the set of edges in $G$. Each statement of $P$ is represented by a node in the ICFG and edges between nodes represent the flow of control in $P$. $E_d\subseteq V\times V$ represent data dependency edges in $G$.
\begin{definition}
Let $G=(V,E,H)$ denote an annotated Inter-procedural Control-Flow Graph (ICFG) of a program $P$.
Each statement of $P$ is represented by a vertex $v \in V$ in $G$, and edges $E\subseteq V\times V$ represent the flow of control in $P$.
% \twr{Move the remainder of the paragraph to Section \ref{sec:problemStmt}, where you can say that you annotate the CFG according to the function (?) $H$. Note that your use of pairs ($v \in V,h$) is not consistent with Eqn.~(\ref{eq:annotation}), where you use $H(v)$.}
% The set of annotations, $H$, is composed of pairs ($v \in V,h$), where $h$ is an annotation of the vertex $v$.
% $h+$ indicates $v$ contains a \emph{configuration-hosting variable}, otherwise the vertex $v$ is assigned the label $h-$.
\end{definition}
% where $V$ is the set of vertices. $E\subseteq V\times V$ is the set of edges in $G$. 



Graph $G$ is said to be a \textit{connected graph} if there is at least one path between every pair of vertices in $G$. Otherwise, $G$ is disconnected.
% \twr{A vertex cut is a set of nodes, not a single node $v$. But I think you can just go directly to define an articulation point.} %ma{yes, this point was confusing me when I was reading different graph theory resources. But I noticed both terms are synonyms.}
A \textit{vertex-cut} on $G$ deletes vertex $v$, which partitions $G$ into two disjoint non-empty sub-graphs.
% \twr{Rephrase properly: ... is a set ... that partitions $G$ into two disjoint non-empty sub-graphs.}
% partition of $E_c$ into subsets by cutting some vertices in $E_c$.
% An \textbf{Articulation Point}
% \twr{Why not ``an articulation point $p$ of $G$ is a vertex such that the singleton set $\{ p \}$ is a vertex cut on $G$.''
%}
Specifically, vertex $v$ in the connected graph $G$ is a cut-vertex if and only if there exist two vertices $x$ and $y$ in $G$ such that every path between $x$ and $y$ passes through $v$~\cite{deo2017graph}. Therefore, 
% \ma{The next stmt might not be fully accurate, because in general there are one or more articulation point. But \name populates only one articulation point} 
vertex $v$ is an \textit{articulation point} $p$ of $G$ such that the singleton set $\{ p \}$ is a vertex cut on $G$. 
% The minimum number of vertices whose deletion causes a connected graph to not be disconnected is known as \textit{vertex-connectivity}.
% \twr{Why do you need to define vertex connectivity?} \ma{old details forget removing them}
% and denoted as $\kappa(G)$.

% \twr{Verbose and poorly worded:}\ma{Agreed. here I was trying }The problem identifying the \neck as vertex cut graph partitioning problem because the \neck represents a physical separation between configuration logic as illustrated in Figure~\ref{fig:illustrativeEx}. In other words, the \neck separates $G$ into two disconnected partitions (configuration logic and main logic). This indicates the \neck should be an articulation point in $G$. However, the \neck is not a typical articulation point, since it captures the stage where run-time-configurations are translated from external format to configuration-hosting variables. Therefore, it is necessary to enrich $G$ by considering $E_d$, data-flow edges that track the use of run-time configurations. 

The next section presents our definition of the {\neck}-identification problem.

\begin{comment}
The next section presents our {\neck}-identification algorithm, which augments the idea of finding an articulation point with the ideas from the Finding in Section~\ref{sec:stucturalProp}.
\end{comment}
